Data and Knowledge for Overtaking Scenarios in Autonomous Driving

Autonomous driving has become one of the most popular research topics within Artificial Intelligence. An autonomous vehicle is understood as a system that combines perception, decision-making, planning, and control. All of those tasks require that the vehicle collects surrounding data in order to make a good decision and action. In particular, the overtaking maneuver is one of the most critical actions of driving. The process involves lane changes, acceleration and deceleration actions, and estimation of the speed and distance of the vehicle in front or in the lane in which it is moving. Despite the amount of work available in the literature, just a few handle overtaking maneuvers and, because overtaking can be risky, no real-world dataset is available. This work contributes in this area by presenting a new synthetic dataset whose focus is the overtaking maneuver. We start by performing a thorough review of the state of the art in autonomous driving and then explore the main datasets found in the literature (public and private, synthetic and real), highlighting their limitations, and suggesting a new set of features whose focus is the overtaking maneuver.

==> acros.tex <==
%------ Acronyms definitions
% http://www.ctan.org/tex-archive/macros/latex/contrib/acronym/
% Place the acronyms in alphabetical order as the acronyms chapter will not order it automatically
\acro{ADAS}{Advanced Driver Assistance Systems}
\acro{AI}{Artificial Intelligence}
\acro{AUC}{Area Under the Curve}
\acro{AV}{Autonomous Vehicle}
\acro{CNN}{Convolutional Neural Networks}
\acro{DNN}{Deep Neural Network}
\acro{ER}{Entity Relationship}
\acro{GAN}{Generative Adversarial Network}
\acro{ILP}{Inductive Logic Programming}
\acro{ITS}{Intelligent Transport Systems}
\acro{KB}{Knowledge Base}
\acro{KR}{Knowledge Representation}
\acro{KRR}{Knowledge Representation and Reasoning}
\acro{LiDAR}{Light Detection and Ranging}
\acro{NHTSA}{National Highway Traffic Safety Administration}
\acrodef{RNN}{Recurrent Neural Network}
\acro{ROC}{Receiver Operating Characteristic}
\acro{ROS}{Robot Operating System}
\acro{SAE}{Society of Automotive Engineers}
\acro{SBS}{Sequential Backward Selection}
\acro{SMOTE}{Synthetic Minority Oversampling TEchnique}
\acro{SVM}{Support Vector Machines}
\acro{YAP}{Yet Another Prolog}



==> tables/comparison_simulators.tex <==
\begin{table}[H]
\caption{Comparison of popular simulators. Adapted from~\cite{survey_simulators}. \\
Legend: Y indicates that simulator has the corresponding requirement; 
N indicates the opposite; (-) indicates that no information is provided. }
\label{tab:survey_simulators}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}|c|c|c|c|c|c|c|c|c|c|c|c|@{}}
\toprule
\rowcolor{blue} 
Requirements & CARLA & CarSim & \begin{tabular}[c]{@{}c@{}} Voyage \\ Deepdrive \end{tabular} & rFpro & AirSim & Deepdrive & Prescan & Gazebo & LGSVL & \begin{tabular}[c]{@{}c@{}} MATLAB \\ (Simulink) \end{tabular} \\ \midrule
Perception: Sensor models supported & Y & Y & Y & Y & Y & Y & Y & Y & Y & Y \\ \midrule
Perception: Support different weather conditions & Y & N & Y & Y & Y & Y & Y & N & Y & N\\ \midrule
Camera Calibration & Y & N & N & Y & N & N & Y & N & N & Y \\ \midrule
Path Planning & Y & Y & Y & Y & Y & Y & Y & Y & Y & Y \\ \midrule
Vehicle Control: Support for proper vehicle dynamics & Y & Y & Y & Y & Y & Y & Y & Y & Y & Y\\ \midrule
3D Virtual Environment & Y & Y & Y & Y & Y & Y & Y & Y & Y & - \\ \midrule
Traffic Infrastructure & Y & Y & Y & Y & Y & Y & Y & Y & Y & Y  \\ \midrule
\begin{tabular}[c]{@{}c@{}} Traffic Scenario simulation: \\ Support of different types of Dynamic objects \end{tabular}
  & Y & Y & Y & Y & Y & Y & Y & N & Y & Y \\ \midrule
2D/3D Ground Truth & Y & N & Y & Y & Y & Y & N & Y & Y & Y \\ \midrule
Interfaces to other software & Y & Y & - & Y & Y & - & Y & Y & Y & Y  \\ \midrule
Scalability via a server multi-client architecture & Y & Y & - & Y & Y & - & - & Y & Y & - \\ \midrule
Open Source & Y & N & Y & Y & Y & Y & N & Y & Y & N \\ \midrule
Well-maintained/Stable & Y & Y & - & Y & Y & - & Y & Y & Y & Y \\ \midrule
Portability & Y & Y & - & Y & Y & Y & Y & Y & Y & Y \\ \midrule
Flexible API & Y & Y & Y & Y & Y & Y & Y & Y & Y & Y \\ \bottomrule
\end{tabular}%
}

\end{table}

==> tables/decision_methods.tex <==
\begin{table}[H]
\caption{Characteristic of different methods for decision-making. Adapted from~\cite{inputs_decision}.}
\label{tab:decision_methods}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|cc|c|c|}
\toprule
\rowcolor{blue} 
\multicolumn{2}{|c|}{Methods}                & Pros & Cons \\ \midrule
\multicolumn{1}{|c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} \\ \\  Classical \\ Methods\end{tabular}}} &
  \begin{tabular}[c]{@{}c@{}}Rule-based \\ Methods\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}
  \tabitem Strong interpretability and adjustability \\ 
  \tabitem Strong feasibility of implementation since its \\ low requirements for hardware \\ 
  \tabitem Good decision-making breadth
  \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}
  \tabitem Difficult to handle complex driving conditions \\ since the lack of decision-making depth \\
  \tabitem Poor robustness for dynamic driving \\ environment
  \end{tabular} \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                   & \begin{tabular}[c]{@{}c@{}} Optimization \\ Methods  \end{tabular} &  
\begin{tabular}[c]{@{}c@{}}
\tabitem Optimized decisions can be generated \\
\tabitem Interaction between different traffic \\
participants can be better modeled
\end{tabular}
   & 
   \begin{tabular}[c]{@{}c@{}}
\tabitem The assumption of "optimal strategy" for agents \\
is often inconsistent with practical applications
\end{tabular}
\\ \cline{2-4} 
\multicolumn{1}{|c|}{}                   & \begin{tabular}[c]{@{}c@{}} Probabilistic \\ Methods \end{tabular} & 
\begin{tabular}[c]{@{}c@{}}
\tabitem Convenient to combine with other types of \\
methods
\end{tabular}
& \begin{tabular}[c]{@{}c@{}}
\tabitem Low computational efficiency and difficult to \\
generate optimal decision in complex \\
environment
\end{tabular}    \\ \midrule
\multicolumn{1}{|c|}{\multirow{3}{*}{ \begin{tabular}[c]{@{}c@{}} \\ \\ \\ \\ Learning-Based \\ Methods \end{tabular}}} & \begin{tabular}[c]{@{}c@{}} Statistic \\ Learning-Based \\ Methods\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}
\tabitem Good versatility \\
\tabitem Suitable for simple scenarios with sufficient \\
environmental information
\end{tabular}
& \begin{tabular}[c]{@{}c@{}}
\tabitem Requirement for plenty of training datasets \\
\tabitem Low decision-making accuracy
\end{tabular}    \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                   & \begin{tabular}[c]{@{}c@{}} Deep \\Learning-Based \\ Method \end{tabular} & 
\begin{tabular}[c]{@{}c@{}}
\tabitem High decision-making accuracy for specific \\
scenarios  \\
\tabitem End-to-end system ensures the full utilize of \\
environmental information
\end{tabular}
& \begin{tabular}[c]{@{}c@{}}
\tabitem Poor universality of algorithms in dynamic \\
scenario. \\
\tabitem Requirement for plenty of training datasets thus \\
quality of the datasets will greatly influence the \\
effect of algorithm
\end{tabular}    \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                   & \begin{tabular}[c]{@{}c@{}} Reinforcement \\
Learning-Based \\ Methods \end{tabular} & 
\begin{tabular}[c]{@{}c@{}}
\tabitem Better modeling of uncertain and dynamic \\
environments \\
\tabitem Flexible framework of algorithms with high \\
expandability 
\end{tabular}
& \begin{tabular}[c]{@{}c@{}}
\tabitem Greatly depends on the establish of reward \\
function \\
\tabitem Poor stability, over-fitting in DRL methods
\end{tabular}    \\ \bottomrule

\end{tabular} %
}

\end{table}





==> tables/knowledge_techniques.tex <==
\begin{table}[H]
\centering
\caption{Advantages and disadvantages of various knowledge representation techniques~\cite{comparision_knowledge} \cite{frames} \cite{semantic_networks} \cite{aima_4th}.}
\label{tab:knowledge_techniques}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|}
\toprule
\rowcolor{blue} 
\begin{tabular}[c]{@{}c@{}}FORMS TO \\ REPRESENT KNOWLEDGE\end{tabular} &
  ADVANTAGES &   DISADVANTAGES \\ \midrule
Semantic Networks &
  \begin{tabular}[c]{@{}c@{}}
  \tabitem It is simple and comprehensible\\ 
  \tabitem Efficient in space requirement\\ 
  \tabitem Easily clusters related knowled\\ 
  \tabitem It is flexible and easy to visualize\\ 
  \tabitem It is a natural representation of knowledge\\ 
  \tabitem Conveys meaning in a transparent manner
  \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}
  \tabitem Take more computational time at runtime\\ 
  \tabitem Inadequate as they do not have any equivalent quantifiers\\ 
  \tabitem Not intelligent and depend on the creator of the system\\ 
  \tabitem It’s difficult to express some properties like negation, disjunction, etc.\\ 
  \tabitem Links on objects represent only binary options\\ 
  \tabitem Inheritance cause problems
  \end{tabular} \\ \midrule
Frame &
  \begin{tabular}[c]{@{}c@{}}
  \tabitem It makes the programming easier by grouping the related data.\\  easy to understand and visualize\\ 
  \tabitem It is very easy to add slots for new attributes and relations\\
  \tabitem It is easy to include default data and search for missing values
  \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}
  \tabitem The mechanism cannot be easily processed\\ 
  \tabitem The inference mechanism cannot be smoothly proceeded by frame \\ representation\\ 
  \tabitem It has a very generalized approach
  \end{tabular} \\ \midrule
Rules &
  \begin{tabular}[c]{@{}c@{}}
  \tabitem Easy to modify and maintain often allow certainty values to be \\ associated with rules and facts\\ 
  \tabitem Easy to understand (natural form of knowledge)\\ 
  \tabitem Easy to derive inference and explanations\\ 
  \tabitem Easy to combine with uncertainty
  \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}
  \tabitem Tend to allow only relatively simple representations of the \\ underlying facts in the domain\\ 
  \tabitem Complex knowledge requires many rules\\ 
  \tabitem Search limitations in systems with many rules
  \end{tabular} \\ \midrule
Logic &
  \begin{tabular}[c]{@{}c@{}}
  \tabitem Helps to perform logical reasoning\\ 
  \tabitem Is the basis for the programming languages
  \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}
  \tabitem Have some restrictions and are challenging to work with\\ 
  \tabitem This technique may not be very natural, and inference may not be \\ very efficient\end{tabular} \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/sensors.tex <==
\setcellgapes{4pt}
\begin{table}[t]
\caption{Comparison of sensors used for autonomous driving. Adapted from~\cite{GRUYER2017323} and~\cite{liu2020computing}.\\ Legend: (++): perfectly adapted sensors; (+): sensors having good performances; (\texttt{-}): sensors potentially meeting the criteria but with possible disadvantages; (\texttt{-{}-}): sensors that can be used with adaptations and additional heavy treatments; (0): sensors unable to meet the criteria.}
\label{tab:sensors_table}
\makegapedcells
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cc|c|c|c|c|c|c|c|@{}} 
\cmidrule(l){3-9}
\multicolumn{2}{c|}{}  
& \cellcolor{blue}Radar short range & \cellcolor{blue}Radar long range & \cellcolor{blue}LiDAR & \cellcolor{blue}Ultrassonic & \cellcolor{blue}Camera & \cellcolor{blue}Camera 3D & \cellcolor{blue}Camera IR \\ \midrule
\multicolumn{2}{|c|}{Range <2m (short range)}  
& - & - & -  & ++ & -- & ++ & -- \\ \midrule                       
\multicolumn{2}{|c|}{Range 2m - 30m (norminal range)}       
& + & ++ & ++  & -- & -- & - & -- \\ \midrule                      
\multicolumn{2}{|c|}{Range >30m - 150m (long range)}                
& n.a & ++ & +  & 0 & -- & -- & -- \\ \midrule  
\multicolumn{2}{|c|}{Field of View angle <10º}                     
& + & + & ++  & -- & ++ & + & ++ \\ \midrule  
\multicolumn{2}{|c|}{Field of View angle >30º}                   
& - & -- & ++  & - & ++ & + & ++ \\ \midrule  
\multicolumn{2}{|c|}{Angular resolution}                           
& - & - & +  & -- & ++ & + & ++ \\ \midrule  
\multicolumn{2}{|c|}{Direct Speed Information}                     
& ++ & ++ & 0 & - & 0 & 0 & 0 \\ \midrule  
\multicolumn{2}{|c|}{Night Vision}    
& ++ & ++ & ++ & ++ & -- & - & ++ \\ \midrule
\multicolumn{2}{|c|}{Sensitivity to Light}    
& ++ & ++ & + & ++ & 0 & 0 & + \\ \midrule
\multicolumn{2}{|c|}{Cost}    
& + & + & - & ++ & + & - & --\\ \midrule
\multicolumn{1}{|c|}{}                           
& under rain & ++ & + & - & - & - & - & - \\ \cmidrule(l){2-9} 
\multicolumn{1}{|c|}{}  
& in fog and snow & ++ & ++ & -  & + & -- & -- & - \\ \cmidrule(l){2-9} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{working:}} 
& with dust & ++ & ++ & - & ++ & 0 & 0 & 0  \\ \midrule
\multicolumn{2}{|c|}{Application Scenarios}   
& \multicolumn{2}{c|} {\shortstack{Object Detection \\ Distance Estimation}}  
& \shortstack{Object Detection \\ Distance Estimation \\ Edge Detection} & \shortstack{Object Detection \\ Distance Estimation} & \multicolumn{3}{c|} {\shortstack{Object Classification \\ Edge Detection \\ Lane Tracking }}  
\\ \bottomrule
\end{tabular}%
}

\end{table}
